Yet Meta Learning Can Adapt Fast, It Can Also Break Easily

Meta learning algorithms have been widely applied in many tasks for efficient learning, such as few-shot image classification and fast reinforcement learning. During meta training, the meta learner develops a common learning strategy, or experience, from a variety of learning tasks. Therefore, during meta test, the meta learner can use the learned strategy to quickly adapt to new tasks even with a few training samples. However, there is still a dark side about meta learning in terms of reliability and robustness. In particular, is meta learning vulnerable to adversarial attacks? In other words, would a well-trained meta learner utilize its learned experience to build wrong or likely useless knowledge, if an adversary unnoticeably manipulates the given training set? Without the understanding of this problem, it is extremely risky to apply meta learning in safety-critical applications. Thus, in this paper, we perform the initial study about adversarial attacks on meta learning under the few-shot classification problem. In particular, we formally define key elements of adversarial attacks unique to meta learning and propose the first attacking algorithm against meta learning under various settings. We evaluate the effectiveness of the proposed attacking strategy as well as the robustness of several representative meta learning algorithms. Experimental results demonstrate that the proposed attacking strategy can easily break the meta learner and meta learning is vulnerable to adversarial attacks. The implementation of the proposed framework will be released upon the acceptance of this paper.

==> sections/intro.tex <==

\section{Introduction}
\label{intro}
Deep neural networks have achieved extraordinary accomplishments in numerous domains such as computer vision~\cite{devlin2018bert} and natural language processing~\cite{krizhevsky2012imagenet}. To achieve satisfying performance, they usually require large-scale training data and heavy hyperparameters tuning. Therefore, learning efficiently and effectively with small data has become one desirable property for modern machine learning techniques. The mechanism of meta-learning (or learn to learn) algorithms~\cite{finn2017model, ravi2016optimization} has been widely used to improve the efficiency of learning new tasks. These meta learning models learn to aggregate prior experience from a set of learning tasks, in order to quickly generalize the experience to new tasks. More specifically, in meta learning, a meta-learner is trained on a distribution of similar tasks (or meta training tasks), with the goal to develop a common learning strategy or the so-called experience for these tasks. During the test time, a meta learner can use its strategy to quickly get the knowledge for a new unseen task (or a meta test task) only based on a few teaching examples. 

Meta learning has already been successfully applied on various tasks such as few shot image classification~\cite{finn2017model} and fast reinforcement learning~\cite{gupta2018meta}. However, there is still a dark side about meta learning -- would a well-trained meta learning model break easily under the threat of a small quantity of malicious perturbations in the training set? In other words, is it possible that the meta learner uses its learned experience to build wrong or almost useless knowledge, if the given training set is unnoticeably manipulated? It is immensely critical and desired to study this problem because without understanding this dark side, it is highly risky to apply it to critical applications pertaining to safety. Imagine in a few-shot image classification task, as shown in Figure~\ref{fig:picture1} and suppose a well-trained meta learner can render a good image classifier when given several training images. If an adversary adds unnoticeable perturbation to one image in the given training set (from $D_{train}^{new}$ to $D_{adv}$), it may mislead the meta learner to produce a classifier with much lower accuracy and even exhibit malicious behaviors. 

%As a consequence, the previous aggregated experience of meta learner can be totally fooled by the adversarially manipulated train set. 

\begin{figure}[h!]
\centering
% \hspace*{-0.8cm} 
%   \includegraphics[width=1\linewidth]{figure/Picture1.pdf}
  \includegraphics[width=1\linewidth]{figure/figure1.png}
  \caption{ For few-shot classification tasks, during the meta test phase, an adversary can insert unnoticeable perturbation to one training sample of $D_{train}$ in the meta test task $\mathcal{T}_{test}$, causing the adapted model which trained on $D_{adv}$ with much lower accuracy. }
    \label{fig:picture1}
\end{figure}

Therefore, we aim to explore this security issue of current popular meta learning algorithms. In this work, we assume that the meta learning system is under the risk of adversaries in the white-box setting \cite{szegedy2013intriguing, goodfellow2014explaining}. In other words, the adversaries have full knowledge of the trained meta learner including its structure and parameters, and the capability to manipulate the input data (e.g., $D_{train}^{new}$ in Figure~\ref{fig:picture1}) of meta learner under certain constraints. 
Then, we evaluate the meta learner's reliability and robustness under these adversarial manipulations. Different from traditional adversarial attacks, we can understand the adversarial attack for meta learning from two perspectives.  From the meta learner perspective, the attack is to generate evasion adversarial examples for the meta test data (e.g., $D_{train}^{new}$ in Figure~\ref{fig:picture1}) during the meta test phase~\cite{szegedy2013intriguing, goodfellow2014explaining}. While from the meta test task (e.g., $\mathcal{T}_{test}$ in Figure~\ref{fig:picture1}) perspective, this attack is to poison its training samples ~\cite{biggio2012poisoning, shafahi2018poison}. To avoid possible confusions, we use the poisoning attack from the meta test task perspective in this work. In fact, we show that comparing with the risks under traditional data poisoning behaviors, the exposure of meta learning models provides the guidance for adversaries to more effectively poison the training data. This will cause more concerns about the data poisoning risks, especially in the systems that require querying training data from external resources such as face recognition~\cite{zhou2018deep}, spam detection~\cite{jindal2007review} and robot imitation learning~\cite{finn2017one}. In summary, our main contributions of this work can be summarized as:
\begin{itemize}
  \item We reveal that meta learning methods learn unreliable experience. These experiences can be fooled by minor poisons which are adversarially inserted into the meta test task. 
  \item We propose an efficient attacking algorithm to generate adversarial inputs for meta learning models under different settings of adversary's capacity and goals, and systematically evaluate their robustness.
  \item We find that for meta test tasks, an adversary is more effective to poison the training samples because of the knowledge of the meta adaptation process, which brings more severe concerns for data poisoning behaviors.
\end{itemize}

\noindent \textbf{Outline of the Paper} The rest of this paper is organized as follows: we introduce preliminary knowledge about meta learning in Section~\ref{meta}. In Section~\ref{threat} we discuss our attacking to meta learning in detail, and present our experimental results in Section~\ref{exp}. We briefly review related work about adversarial attacks and meta learning in Section~\ref{rel}. Finally we conclude our work with future work in Section 6. 
